Pitfalls of Graph Neural Network Evaluation

Semi-supervised node classification in graphs is a fundamental problem in graph mining, and the recently proposed graph neural networks (GNNs) have achieved unparalleled results on this task. Due to their massive success, GNNs have attracted a lot of attention, and many novel architectures have been put forward. In this paper we show that existing evaluation strategies for GNN models have serious shortcomings. We show that using the same train/validation/test splits of the same datasets, as well as making significant changes to the training procedure (e.g. early stopping criteria) precludes a fair comparison of different architectures. We perform a thorough empirical evaluation of four prominent GNN models and show that considering different splits of the data leads to dramatically different rankings of models. Even more importantly, our findings suggest that simpler GNN architectures are able to outperform the more sophisticated ones if the hyperparameters and the training procedure are tuned fairly for all models.

==> chapters/background.tex <==
\section{Semi-supervised node classification}
\label{sec:background}
Given is an undirected unweighted graph $G = (V, E)$ with $N = |V|$ nodes and $M = |E|$ edges,
that can be represented by a symmetric adjacency matrix $\mA \in \{0, 1\}^{N \times N}$.
Every node is associated with a $D$-dimensional attribute vector, represented as an attribute matrix $\mX \in \R^{N \times D}$.
Given a set of labeled nodes $V_L \subset V$, the goal is to predict labels for the unlabeled nodes $V_U = V \setminus V_L$.

\todo{This should be merged with another seciton}

==> figures/planetoid_splits_inverse_ranking.tex <==
% Table contents auto-generated by generate_tables.ipynb
\begin{table}
    \begin{center}
        \begin{tabular}{l C{2cm} C{2cm} C{2cm}}
              & \textbf{\cora} & \textbf{\citeseer} & \textbf{\pubmed} \\
            \midrule
            \textbf{\gcn} & $\textbf{79.0} \pm 0.7$ & $\textbf{68.6} \pm 1.1$ & $69.5 \pm 1.0$ \\
            \textbf{\gat} & $77.9 \pm 0.7$ & $67.7 \pm 1.2$ & -- \\
            \textbf{\monet} & -- & -- & -- \\
            \textbf{\gsmean} & -- & -- & -- \\
            \textbf{\gsmaxpool} & $74.5 \pm 0.6$ & $63.1 \pm 1.2$ & $\textbf{70.3} \pm 0.8$ \\
            \textbf{\gsmeanpool} & -- & -- & -- \\
        \end{tabular}
    \end{center}
    \caption{Another random split with a different best performing model on the raw data introduced by \citet{planetoid}.}
\label{table:planetoid_inverted}
\end{table}

==> figures/planetoid_splits_mean.tex <==
% Table contents auto-generated by generate_tables.ipynb
\begin{table}[h!]
    \begin{center}
        \begin{tabular}{l C{1.6cm} C{1.6cm} C{1.6cm}}
              & \textbf{\cora} & \textbf{\citeseer} & \textbf{\pubmed} \\
            \midrule
            \textbf{\gcn} & $81.9 \pm 0.8$ & $69.5 \pm 0.9$ & $\textbf{79.0} \pm 0.5$ \\
            \textbf{\gat} & $\textbf{82.8} \pm 0.5$ & $\textbf{71.0} \pm 0.6$ & $77.0 \pm 1.3$ \\
            \textbf{\monet} & $82.2 \pm 0.7$ & $70.0 \pm 0.6$ & $77.7 \pm 0.6$ \\
            \textbf{\gsmean} & $77.8 \pm 15.3$ & $70.5 \pm 0.8$ & $78.9 \pm 0.5$ \\
            \textbf{\gsmaxpool} & $77.4 \pm 1.0$ & $67.0 \pm 1.0$ & $76.6 \pm 0.8$ \\
            \textbf{\gsmeanpool} & $78.3 \pm 0.9$ & $66.3 \pm 1.0$ & $75.9 \pm 0.5$ \\
        \end{tabular}
    \end{center}
    \caption{Test set accuracy of all models in percent on the single split introduced by \citet{planetoid} averaged over $20$ different weight initializations. For each dataset, the highest accuracy score is marked in \textbf{bold}. Note that these results do not exactly match the results in the reference papers since we used the optimized hyperparameters as well as our training framework.}
\label{table:planetoid_splits_mean}
\end{table}
